Model-based Outdoor Performance Capture

We propose a new model-based method to accurately reconstruct human performances captured outdoors in a multi-camera setup. Starting from a template of the actor model, we introduce a new unified implicit representation for both, articulated skeleton tracking and nonrigid surface shape refinement. Our method fits the template to unsegmented video frames in two stages - first, the coarse skeletal pose is estimated, and subsequently non-rigid surface shape and body pose are jointly refined. Particularly for surface shape refinement we propose a new combination of 3D Gaussians designed to align the projected model with likely silhouette contours without explicit segmentation or edge detection. We obtain reconstructions of much higher quality in outdoor settings than existing methods, and show that we are on par with state-of-the-art methods on indoor scenes for which they were designed

==> figures/overlap_evaluation/skirt/myfile.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
unbounded coords=jump,
xmin=0,
xmax=80,
ymin=0.9,
ymax=0.99,
axis background/.style={fill=white},
title style={font=\bfseries},
title={Precision},
axis x line*=bottom,
axis y line*=left,
legend style={at={(0.144,0.124)},anchor=south west,legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=mycolor1,solid,line width=2.0pt]
  table[row sep=crcr]{%
1	0.974074074074074\\
2	0.973243254136187\\
3	0.973759069504234\\
4	0.973564608369234\\
5	0.975177943387758\\
6	0.975416612938705\\
7	0.974184559286504\\
8	0.975571947694634\\
9	0.974635288998844\\
10	0.975282380611928\\
11	0.97303839901453\\
12	0.975907396110454\\
13	0.974645228073994\\
14	0.975092936802974\\
15	0.974918673316481\\
16	0.974618130920746\\
17	0.974730362230362\\
18	0.975344105326152\\
19	0.973595608790581\\
20	0.974468356855483\\
21	0.974266062569191\\
22	0.974233346807103\\
23	0.974311555914714\\
24	0.972309749372914\\
25	0.973373278229681\\
26	0.975251829746968\\
27	0.97422230550945\\
28	0.973524729500013\\
29	0.974468886257347\\
30	0.97340357223851\\
31	0.973485128306151\\
32	0.974689134921306\\
33	0.975006659454523\\
34	0.974728920056404\\
35	0.973338365525887\\
36	0.974687962284312\\
37	0.975006450641839\\
38	0.974132129886776\\
39	0.974265324266526\\
40	0.975452984170516\\
41	0.977470541690725\\
42	0.977751563991093\\
43	0.977152816413058\\
44	0.977971523717125\\
45	0.977301643055068\\
46	0.977025105973472\\
47	0.976730962690811\\
48	0.976780727595114\\
49	0.976566994720255\\
50	0.977573896430978\\
51	0.976648545608585\\
52	0.975675783569614\\
53	0.973593027224017\\
54	0.9751810928169\\
55	0.972386719503688\\
56	0.971639832507667\\
57	0.973381615516601\\
58	0.972646252788887\\
59	0.969695272920263\\
60	0.971202934187517\\
61	0.967582866057155\\
62	0.966302654353144\\
63	0.964447412450518\\
64	0.968601742430777\\
65	0.968479087270658\\
66	0.967756652908175\\
67	0.966498329651701\\
68	0.964623329912341\\
69	0.966661856991809\\
70	0.967268198971165\\
71	0.96527993815813\\
72	0.966573224600748\\
73	0.966763488920768\\
74	0.96602442719182\\
75	0.967726035617084\\
76	0.966538891931145\\
77	0.966405637465818\\
78	0.967228919121288\\
79	0.965634594045311\\
80	0.967859123014247\\
};
\addlegendentry{Jurguen};

\addplot [color=mycolor2,solid,line width=2.0pt]
  table[row sep=crcr]{%
1	0.972765760317072\\
2	0.972729821276552\\
3	0.970889385319757\\
4	0.97144303381151\\
5	0.969979415778153\\
6	0.971706502184528\\
7	0.970916967286406\\
8	0.972135371134127\\
9	0.971369943326168\\
10	0.972488509014026\\
11	0.970965593328001\\
12	0.971763574264963\\
13	0.971321387771065\\
14	0.972188325429803\\
15	0.971494950379526\\
16	0.971838757419335\\
17	0.970643040013214\\
18	0.970922046281871\\
19	0.968974779381102\\
20	0.968284119483391\\
21	0.965554205488327\\
22	0.962796317996873\\
23	0.959263021746985\\
24	0.956318018915799\\
25	0.950291609164406\\
26	0.945860787924593\\
27	0.939791347400684\\
28	0.939760273787447\\
29	0.937304706638069\\
30	0.934314925303976\\
31	0.932820885646836\\
32	0.935170808509018\\
33	0.935346243988018\\
34	0.937836740219304\\
35	0.936504639059832\\
36	0.939939948019522\\
37	0.939927316484868\\
38	0.940395292503591\\
39	0.939528429765766\\
40	0.939339142309241\\
41	0.936889938285884\\
42	0.939939192338658\\
43	0.939717592604796\\
44	0.940782831924774\\
45	0.940618573897088\\
46	0.940119527795264\\
47	0.937465879711175\\
48	0.936270318699603\\
49	0.934803085461164\\
50	0.935045558288518\\
51	0.932865102705809\\
52	0.932812276819835\\
53	0.9309737779152\\
54	0.932035049201011\\
55	0.929522168670523\\
56	0.92995033267735\\
57	0.927851553964641\\
58	0.924331565808771\\
59	0.921626979318635\\
60	0.919503891050584\\
61	0.915181265265073\\
62	0.913734946642259\\
63	0.907413191733042\\
64	0.910498248684455\\
65	0.909071573647959\\
66	0.907174398839186\\
67	0.905946502105295\\
68	0.905006649673058\\
69	0.904017373921615\\
70	0.905733254810302\\
71	0.903932551960525\\
72	0.903385111034403\\
73	0.903181218165357\\
74	0.905971479500891\\
75	0.90605630509126\\
76	0.907030557347828\\
77	0.905567264808971\\
78	0.906852305958862\\
79	0.904997981277523\\
80	0.905550984030576\\
};
\addlegendentry{Stage I};

\addplot [color=mycolor3,solid,line width=2.0pt]
  table[row sep=crcr]{%
1	nan\\
2	nan\\
3	nan\\
4	nan\\
5	nan\\
6	nan\\
7	nan\\
8	nan\\
9	nan\\
10	nan\\
11	nan\\
12	nan\\
13	nan\\
14	nan\\
15	nan\\
16	nan\\
17	nan\\
18	nan\\
19	nan\\
20	nan\\
21	0.970095417473658\\
22	0.969087516641169\\
23	0.968864253161964\\
24	0.967878143053928\\
25	0.964275924843683\\
26	0.961573776632133\\
27	0.958349569778096\\
28	0.96091041538167\\
29	0.957618729527657\\
30	0.955840482700104\\
31	0.957694074414332\\
32	0.957153412467674\\
33	0.957552765161635\\
34	0.95779138110293\\
35	0.953629010970446\\
36	0.953717415506123\\
37	0.954321587580935\\
38	0.955464112073597\\
39	0.955538789603014\\
40	0.957221624669751\\
41	0.955799794623729\\
42	0.959879823519958\\
43	0.960370604881957\\
44	0.960729704454323\\
45	0.960347642688118\\
46	0.958677811089912\\
47	0.95734949503068\\
48	0.957250448714268\\
49	0.957436118110295\\
50	0.958092428420356\\
51	0.95868857312019\\
52	0.96034676000118\\
53	0.95924616561409\\
54	0.960199637289743\\
55	0.958475460003119\\
56	0.95742414758529\\
57	0.956644752459898\\
58	0.954571899777379\\
59	0.952647761558869\\
60	0.950560778296621\\
61	0.949509003191004\\
62	0.947398609255579\\
63	0.942801532581495\\
64	0.944461302882326\\
65	0.943920520567046\\
66	0.942218252237156\\
67	0.940198563679777\\
68	0.938655948538343\\
69	0.937451672088544\\
70	0.937547675709255\\
71	nan\\
72	nan\\
73	nan\\
74	nan\\
75	nan\\
76	nan\\
77	nan\\
78	nan\\
79	nan\\
80	nan\\
};
\addlegendentry{Silhouette Outter};

\addplot [color=mycolor4,solid,line width=2.0pt]
  table[row sep=crcr]{%
1	nan\\
2	nan\\
3	nan\\
4	nan\\
5	nan\\
6	nan\\
7	nan\\
8	nan\\
9	nan\\
10	nan\\
11	nan\\
12	nan\\
13	nan\\
14	nan\\
15	nan\\
16	nan\\
17	nan\\
18	nan\\
19	nan\\
20	nan\\
21	0.965454695784284\\
22	0.963163431343082\\
23	0.961401272228221\\
24	0.958519175811987\\
25	0.953113260582879\\
26	0.951855019581571\\
27	0.948074293497312\\
28	0.949349662322067\\
29	0.945965840567585\\
30	0.942193436866395\\
31	0.943268147705837\\
32	0.945830141643366\\
33	0.946614396755661\\
34	0.947808455309914\\
35	0.945631598253228\\
36	0.947579955989489\\
37	0.947088129644867\\
38	0.947341317873904\\
39	0.947668556022587\\
40	0.947984574297731\\
41	0.94519706381767\\
42	0.949156013453374\\
43	0.949971720641837\\
44	0.951681071635969\\
45	0.952201192636764\\
46	0.952795906929655\\
47	0.951603374226825\\
48	0.951032112434376\\
49	0.950367698459301\\
50	0.952151944350686\\
51	0.950722552471824\\
52	0.951665405662203\\
53	0.950312471832467\\
54	0.950493043867525\\
55	0.948665128748675\\
56	0.948592453919919\\
57	0.947372740566835\\
58	0.945604095039369\\
59	0.944075042727465\\
60	0.941827281049741\\
61	0.940387376207509\\
62	0.936664002388221\\
63	0.931322274187781\\
64	0.935705915065361\\
65	0.933121305911963\\
66	0.930652505221171\\
67	0.928795978317396\\
68	0.928315638249413\\
69	0.9262103816865\\
70	0.925455004528618\\
71	0.922851100537051\\
72	0.923075137908708\\
73	0.922446787237308\\
74	0.924659658154332\\
75	0.92431177104796\\
76	0.925105722617608\\
77	0.923814321833993\\
78	0.924702321936111\\
79	0.924183978375605\\
80	0.924928763040238\\
};
\addlegendentry{Inner only};

\addplot [color=mycolor5,solid,line width=2.0pt]
  table[row sep=crcr]{%
1	nan\\
2	nan\\
3	nan\\
4	nan\\
5	nan\\
6	nan\\
7	nan\\
8	nan\\
9	nan\\
10	nan\\
11	nan\\
12	nan\\
13	nan\\
14	nan\\
15	nan\\
16	nan\\
17	nan\\
18	nan\\
19	nan\\
20	nan\\
21	0.98305953425987\\
22	0.982234384620647\\
23	0.981643024899484\\
24	0.980887934299164\\
25	0.977776849143335\\
26	0.974000506428833\\
27	0.972169700847133\\
28	0.973652134229118\\
29	0.974971439229675\\
30	0.97446329134612\\
31	0.973385990511223\\
32	0.972120033100565\\
33	0.970283815989023\\
34	0.972262546661136\\
35	0.968910047090365\\
36	0.970939673353139\\
37	0.969507707608155\\
38	0.971227284325121\\
39	0.971039566934134\\
40	0.97040548098434\\
41	0.969950642759544\\
42	0.972289526953122\\
43	0.972199522947127\\
44	0.97196052896849\\
45	0.971785237299293\\
46	0.97135040513765\\
47	0.968628464956591\\
48	0.96888962917136\\
49	0.967947538570715\\
50	0.968419923443824\\
51	0.96786159609112\\
52	0.968554109955839\\
53	0.970070755511339\\
54	0.968163588906679\\
55	0.966768372551739\\
56	0.9651165162929\\
57	0.963661778547542\\
58	0.961102271487265\\
59	0.960149783508106\\
60	nan\\
61	nan\\
62	nan\\
63	nan\\
64	nan\\
65	nan\\
66	nan\\
67	nan\\
68	nan\\
69	nan\\
70	nan\\
71	nan\\
72	nan\\
73	nan\\
74	nan\\
75	nan\\
76	nan\\
77	nan\\
78	nan\\
79	nan\\
80	nan\\
};
\addlegendentry{Outer only};

\addplot [color=mycolor6,solid,line width=2.0pt]
  table[row sep=crcr]{%
1	nan\\
2	nan\\
3	nan\\
4	nan\\
5	nan\\
6	nan\\
7	nan\\
8	nan\\
9	nan\\
10	nan\\
11	nan\\
12	nan\\
13	nan\\
14	nan\\
15	nan\\
16	nan\\
17	nan\\
18	nan\\
19	nan\\
20	nan\\
21	0.981457444334474\\
22	0.980842662324445\\
23	0.979606347476674\\
24	0.979876228932584\\
25	0.976997076976632\\
26	0.972828691475253\\
27	0.970743508291977\\
28	0.971248386986262\\
29	0.97261806822039\\
30	0.973594671565314\\
31	0.972148154981018\\
32	0.972508264783821\\
33	0.970849408151184\\
34	0.971717976441131\\
35	0.96827674835963\\
36	0.971591037363134\\
37	0.970490349592264\\
38	0.972270373673965\\
39	0.971179491485104\\
40	0.972138966280649\\
41	0.971166419183972\\
42	0.972205766192733\\
43	0.972314029270211\\
44	0.972286617777141\\
45	0.971168278405558\\
46	0.971678587125904\\
47	0.969827038362955\\
48	nan\\
49	nan\\
50	nan\\
51	nan\\
52	nan\\
53	nan\\
54	nan\\
55	nan\\
56	nan\\
57	nan\\
58	nan\\
59	nan\\
60	nan\\
61	nan\\
62	nan\\
63	nan\\
64	nan\\
65	nan\\
66	nan\\
67	nan\\
68	nan\\
69	nan\\
70	nan\\
71	nan\\
72	nan\\
73	nan\\
74	nan\\
75	nan\\
76	nan\\
77	nan\\
78	nan\\
79	nan\\
80	nan\\
};
\addlegendentry{Inner and Outer};

\end{axis}
\end{tikzpicture}%
